Convergence of online $k$-means

We prove asymptotic convergence for a general class of $k$-means algorithms performed over streaming data from a distribution: the centers asymptotically converge to the set of stationary points of the $k$-means cost function. To do so, we show that online $k$-means over a distribution can be interpreted as stochastic gradient descent with a stochastic learning rate schedule. Then, we prove convergence by extending techniques used in optimization literature to handle settings where center-specific learning rates may depend on the past trajectory of the centers.

==> sections/body.tex <==
%!TEX root = ../main.tex

\section{Preliminaries} \label{sec:prelim}
Let $p$ be a density on $\mathbb{R}^d$ with bounded second moment. Notice that because $p$ is a density, any Lebesgue measure zero set also has zero probability mass. We denote a tuple of $k$ centers or prototypes in $\mathbb{R}^d$ by $w = \big(w_1,\ldots, w_k\big) \in \mathbb{R}^{k \times d}$. Define the following:
\renewcommand\labelitemi{$\vcenter{\hbox{\tiny$\bullet$}}$}
\begin{itemize}
    \item $V(w) = \big(V_1(w),\ldots, V_k(w)\big)$ is the induced Voronoi partitioning\footnote{Strictly speaking, $V(w)$ does not partition $\mathbb{R}^{k \times d}$ because adjacent partitions $V_i(w)$ and $V_j(w)$ share boundary points. However, boundary points form a measure zero set, so we will encounter no problems.}
    of $\mathbb{R}^d$ by $w$
    \[V_i(w) = \bigg\{x \in \mathbb{R}^d : w_i \in \argmin_{w_j} \,\|w_j - x\|\bigg\}\]
    \item $P(w) = \big(P_1(w),\ldots, P_k(w)\big)$ is the probability mass of each of the Voronoi partitions
    \[P_i(w) = \int_{V_i(w)} p(x)\,dx\]
    \item $M(w) = \big(M_1(w),\ldots, M_k(w)\big)$ is the mean/center of mass of each of the Voronoi partitions
    \[M_i(w) = \frac{1}{P_i(w)} \int_{V_i(w)} x\, p(x)\,dx.\]
\end{itemize}
While these functions are defined for all $w \in \mathbb{R}^{k \times d}$, we will be able to restrict our analysis to the set of non-degenerate tuples, where none of the centers coincides:
\[\mathcal{D} := \{w \in \mathbb{R}^{k \times d} : w_i \ne w_j, \ \forall i\ne j\}.\]
Later on, we will restrict the support of $p$ to a closed ball $B(0,R)$ centered at the origin of radius $R$ in $\mathbb{R}^d$. Let $\mathcal{D}_R$ be the set of non-degenerate tuples in $B(0,R)$:
\[\mathcal{D}_R := \{w \in \mathcal{D} : w_i \in B(0,R), \ \forall i \in [k]\}.\]
As last bits of notation, given a Borel set $S \subset \mathbb{R}^d$ with positive probability mass $p(S) > 0$, let $p\big|_S$ denote the distribution obtained by restricting $p$ onto $S$. Finally, we will also let $[k]$ denote the set $\{1,\ldots, k\}$.

\paragraph{The \textit{k}-means problem}
The $k$-means objective is to minimize:
\begin{equation}\label{eqn:kmeans-cost}
f(w) := \frac{1}{2}\sum_{i \in [k]}\ \int_{V_i(w)} \| w_i - x\|^2\, p(x) \,dx.
\end{equation} 
While the $k$-means cost is non-convex, we show that it is smooth on $\mathcal{D}$. Therefore, we aim for convergence to stationary points---the iterates $W^{(n)}$ approach the set of stationary points $\{\nabla f = 0\}$ in the limit as $n \to \infty$. 

\begin{definition}[Global convergence]
Let $\mathcal{D}$ be a domain and $f : \mathcal{D} \to \mathbb{R}$ be differentiable. We say that a sequence of points $(w^{(n)})_{n=0}^\infty$ in $\mathcal{D}$ \emph{globally converges to stationary points of $f$} if all limit points of $(w^{(n)})_{n=0}^\infty$ are contained in the set of stationary points $\{\nabla f = 0\}$,
\[\bigcap_{n \geq 0} \overline{(w^{(n')})_{n' \geq n}} \subset \{\nabla f = 0\}.\]
\end{definition}

\section{Main Results}
This section is structured as follows. We will first prove the asymptotic convergence result for a general class of online $k$-means algorithms under some assumptions. Then, we will show that \ref{alg:onlinelloyd} satisfies those assumptions and therefore proving its convergence.

\subsection{Convergence of online $k$-means algorithms}

\subsubsection{Gradient of $k$-means objective}
Computing the derivative of the $k$-means cost (\ref{eqn:kmeans-cost}) with respect to $w$ is relatively involved because the both the domain of integration and the integrand depend on $w$. 

\begin{restatable}[Gradient of $k$-means objective]{lemma}{kmeansgrad} \label{lem:k-means-grad}
Let $p$ be a density on $\mathbb{R}^d$ with $\E_{X \sim p}\left[\|X\|^2\right] < \infty$. Let $f$ be the $k$-means objective (\ref{eqn:kmeans-cost}). Then $f$ is continuously differentiable on $\mathcal{D}$, where:
\begin{align} \label{eqn:grad-f}
    \nabla_{w_i}\, f(w) &= P_i(w) \cdot \big(w_i - M_i(w)\big).
\end{align}
\end{restatable}

\subsubsection{Convergence of cost}
Notice that for the $k$-means objective to be finite, $p$ must have bounded second moment. But for our convergence analysis, we will make a stronger assumption: 
\begin{assumption} \label{assume:finite}
Assume $p$ has bounded support, i.e. $\displaystyle\Pr_{X \sim p}(\|X\| > R ) = 0$ for some $R > 0$.
\end{assumption}
We also make assumptions on the learning rates used in Algorithm~\ref{alg:distributional-kmeans}. Let $X^{(n)}$ and $H^{(n)}$ denote the tuples $\big(X_1^{(n)},\ldots, X_k^{(n)}\big)$ and $\big(H_1^{(n)},\ldots, H_k^{(n)}\big)$, respectively.

\begin{assumption} \label{assume:lr}
Define $\big(\mathcal{F}_n\big)_{n=0}^\infty$ to be the natural filtration associated to the \ref{alg:distributional-kmeans} algorithm. In particular, let $\mathcal{F}_0 = \sigma\big(W^{(0)}\big)$ be the $\sigma$-algebra generated by $W^{(0)}$. Define $\mathcal{F}_n = \sigma\big(X^{(n)}, H^{(n)}, \mathcal{F}_{n-1}\big)$ as the $\sigma$-algebra containing all information up to iteration $n$. We assume that:
\begin{enumerate}
    \item[(1)] If $P_i(W^{(n)}) = 0$, then $H_i^{(n+1)} = 0$ almost surely.
    \item[(2)] $H^{(n+1)}$ and $X^{(n+1)}$ are conditionally independent given $\mathcal{F}_n$.
    \item[(3)] $0 \leq H_i^{(n+1)}\leq 1$.
\end{enumerate}
\end{assumption}

When $P_i(W^{(n)}) = 0$, it may not be sensible to draw from $V_i(W^{(n)})$. The first assumption avoids this situation; we require ${H_i}^{(n+1)} = 0$ a.s.\@ and let ${X_i}^{(n+1)}$ be arbitrary---it is not used to update the centers. The second assumption ensures that $H^{(n+1)}$ does not depend on $X^{(n+1)}$. The final assumption that $H_i^{(n+1)} \leq 1$ is not strictly necessary, but is simplifying for analysis and is intuitively natural: the update is a convex combination of the previous center and new data point.

We do not lose much for making this assumption, and at any rate, we shall require the learning rate to converge to zero in our convergence analysis. From now on, we implicitly make Assumptions \ref{assume:finite} and \ref{assume:lr}.

We now prove the asymptotic convergence of the $k$-means cost, $f(W^{(n)})$, which will be based on a supermartingale argument commonly used in proving the convergence of stochastic gradient descent. Recall that a bounded and monotonically decreasing real-valued sequence converges to a real value. This remains true in the random setting. A supermartingale is a noisy sequence that in expectation decreases monotonically. Provided that the noise can be controlled, then the \emph{martingale convergence theorem} shows that such a stochastic sequence will converge to some real-valued random variable, e.g.\@ see \cite{durrett2019probability}. 


\begin{restatable}[Convergence of cost]{proposition}{propcostconv}
\label{prop:cost-conv}
Let $\big(W^{(n)}\big)_{n=0}^\infty$ be a sequence generated by the \ref{alg:distributional-kmeans} algorithm. If the following series converges:
\[\quad\sum_{n=1}^\infty \sum_{i \in [k]} \big(H_i^{(n)}\big)^2 < \infty \quad \mathrm{a.s.},\]
then there is an $\mathbb{R}$-valued random variable $f^*$ such that $f(W^{(n)})$ converges to $f^*$ almost surely.
\end{restatable}

\subsubsection{Convergence of iterates}
Our main result is the convergence of the $k$-means iterates $W^{(n)}$ to the set of stationary point $\{\nabla f = 0\}$. For this, we need some additional assumption besides Assumptions \ref{assume:finite} and \ref{assume:lr}. Lemmas \ref{lem:non-degenerate} and \ref{lem:lr-iterates-bound} show that the iterates $W^{(n)}$ are non-degenerate and bounded, where $W^{(n)} \in \mathcal{D}_R \subset B(0,R)$. From now on, we restrict all sets to the (topological) subspace $\mathcal{D}_R \subset \mathbb{R}^{k \times d}$. For example, when we write $\{\nabla f = 0\}$, we implicitly mean $\{\nabla f = 0\} \cap \mathcal{D}_R$. We assume:

\begin{assumption}\label{assume:compact-stationary}
The set $\{\nabla f = 0\}$ of stationary points is compact in $\mathcal{D}_R$.
\end{assumption}

Geometrically, this means that $\{\nabla f = 0\}$ has no degenerate limit point (see \Cref{lem:compact-eps}'s proof). This lets us prove that $W^{(n)}$ converges to $\{\nabla f = 0\}$ by showing that $\nabla f(W^{(n)})$ converges to zero. Formally, we apply \Cref{lem:top-conv}, which relies on (i) the continuity of $\nabla f$, and (ii) the existence of a compact subset of $\mathcal{D}_R$ containing $\{\nabla f = 0\}$.

From here on, we additionally make \Cref{assume:compact-stationary}.

The key idea is to link the convergence of $\nabla f(W^{(n)}) \to 0$  to that of $f(W^{(n)}) \to  f^*$. Broadly speaking, we need conditions on the learning rate so that whenever $\|\nabla f(W^{(n)})\|$ is larger than $\epsilon$, then the cost is likely to decrease by at least $\delta$. Then, Borel-Cantelli (\Cref{lem:borel-cantelli}) would show that the cost decreases by a large amount infinitely often if the gradient is large infinitely often. But as the cost converges, this cannot happen.

Were we in the noiseless gradient descent setting, we could---in a single step---turn a large gradient into a large decrease in cost. We simply ensure that the iterates move in a direction that significantly decreases $f$ by lower bounding the learning rates for centers $i \in [k]$ with large gradients $\nabla_{w_i} f$.  However, in our setting, the true gradient direction is obscured by the presence of noise, and so lower bounding the learning rates by a constant no longer guarantees a decrease in cost.

Instead, in the stochastic gradient descent setting, we can---over many steps---turn a \emph{region} with large gradients into a large decrease in cost, with high probability. Since our learning rate decays to zero, eventually, whenever we enter a region with large gradients, we remain in that region for sufficiently many iterations so as to average out the noise and recover the underlying signal to move along the negative gradient direction. As in the noiseless setting, we want the choice of learning rate to not disproportionately dampen learning for centers $i \in [k]$ with large gradients $\nabla_{w_i} f$. In other words, the iterates should not leave this region of large gradients before having accumulated enough learning on those centers with large gradients. 

As a motivating adversarial example, suppose we decrease the learning rates for centers with large gradients while increasing the rates for centers with small gradients. Then, the iterates may escape the region with large gradients by moving orthogonally to the gradient descent direction, not significantly decreasing the function value. And as an extreme example, if we never update the $i$th center, so $H_i^{(n+1)} \equiv 0$ for all $n$, then the cost $f(W^{(n)})$ may converge while the gradients $\|\nabla f(W^{(n)})\|$ may never converge to zero. 

To preclude these examples, we need to be able to control the learning rates whenever the gradient $\|\nabla_{w_i} f(W^{(m)})\|$ becomes large for center $i \in [k]$ at iteration $m$. But because the convergence of cost analysis required the learning rates to decay to zero (\Cref{prop:cost-conv}), to accumulate the same amount of learning, we will need to control the learning rates over increasingly many iterations as $m \to \infty$. In particular, if the gradient becomes large at iteration $m$, we shall aim to control the learning rates during the interval between $m$ and a future horizon $T(m)$, for some appropriately chosen function $T : \mathbb{N} \to \mathbb{N}$.

We impose two types of conditions on the learning rate. The first condition allows us to ensure that the iterates remain within the region of large gradients during the interval from $m$ to $T(m)$. Recall \Cref{lem:lr-iterates-bound} showed that we can bound the total displacement between $W^{(m)}$ and $W^{(T(m))}$ by bounding the accumulated learning rates; the first condition is of the form:
\[\sum_{j \in [k]} \sum_{m \leq n < T(m)} H_j^{(n+1)} < r.\]
 The second condition ensures that we accumulate enough learning for the center $i \in [k]$ with large gradients, so that the cost decreases by a constant between iterations $m$ and $T(m)$,
\[\sum_{m \leq n < T(m)} H_i^{(n+1)} > s.\]
In fact, it is enough that these conditions hold with constant probability.


\begin{restatable}[Convergence of iterates]{theorem}{thmiteratesconv}  \label{thm:iterates-conv-simple}
Let $W^{(n)}$ and $H^{(n+1)}$ be as in \Cref{prop:cost-conv}. Suppose that for all $i \in [k]$, $\epsilon > 0$, and sufficiently small $r > 0$, there exists $T : \mathbb{N} \to \mathbb{N}$, $m_0 \in \mathbb{N}$, and some $s, c > 0$ so that:
\begin{align*}
&\Pr\Bigg(\sum_{j \in [k]}\sum_{m \leq n < T(m)}  H_j^{(n+1)}  < r \quad \mathrm{and} \sum_{m \leq n < T(m)} H_i^{(n+1)} > s 
\, \Bigg|\, \mathcal{F}_m, \|\nabla_{w_i} f(W^{(m)})\| > \epsilon \Bigg) > c,
\end{align*}
for any $m > m_0$. Then, $W^{(n)}$ globally converges to stationary points of the $k$-means cost $f$ almost surely.
\end{restatable}
We prove a slightly more general theorem in \Cref{thm:iterates-conv}, which makes the decomposition (\ref{eqn:dr-break}) explicit. We introduce separate conditions on the learning rate on $\{\|\nabla_{w_i} f\| \in [\epsilon,\epsilon_0]\}$ and $\{\|\nabla_{w_i} f\| > \epsilon_0\}$; that way, we can remove the learning rate upper bound condition where we do not need it.

\subsection{Convergence of Online Lloyd's algorithm}
Let us return now to extending Lloyd's algorithm into the online setting.
Lloyd's algorithm is defined to iteratively set each center $w_i$ to $M_i(w)$,
\[w_i \leftarrow  M_i(w).\]
Since $\nabla_{w_i} f(w) = P_i(w) \cdot \big(w_i - M_i(w)\big)$, the Lloyd update is precisely \textit{preconditioned gradient descent}, where the preconditioner at $w$ for the $i$th center is $P_i(w)^{-1}$. 
\begin{equation*}  \label{eqn:batch-update}
w_i \leftarrow w_i - \frac{1}{P_i(w)} \nabla_{w_i} f(w).
\end{equation*}
A noiseless gradient descent algorithm is often converted into a stochastic one by introducing decaying learning rates, which allows the noise to average out over time \citep{bottou1998online}. Applying the common decay rate of $n^{-1}$, we might aim for an update that, in expectation, looks like:
\[w_i \leftarrow w_i - \frac{1}{n P_i(w)} \nabla_{w_i} f(w).\]

As a first pass at designing the stochastic version of Lloyd's algorithm, suppose that we had access directly to $p$. Then, we might consider the following idealized learning rate achieving the above expected update:
\[H_{\mathrm{ideal},i}^{(n+1)} \leftarrow  \frac{\ind\{I^{(n+1)} = i\}}{nP_i(W^{(n)})},\]
where $I^{(n+1)}$ is the index of the updated center; it is drawn from the distribution $P(W^{(n)})$ over $[k]$. Naive Lloyd's algorithm described in \Cref{sec:motivation} could then be considered as a rough approximation to this idealized learning rate. To compare, recall the naive Lloyd's update:
\begin{equation*}
H_{\mathrm{naive},i}^{(n+1)} \leftarrow \frac{\ind\{I^{(n+1)} = i\}}{N_i^{(n)} + 1},
\end{equation*}
where $N_i^{(n)}$ is the update count for the $i$th center. If $P(W^{(n)})$ does not vary much over time, then $N_i^{(n)} + 1$ is approximately equal to $nP_i(W^{(n)})$. In other words, the naive Lloyd's update appears to approximate the idealized learning rate by applying a stochastic preconditioner computed on:
\[\widehat{P}_i^{(n)} = \frac{N_i^{(n)}}{n}.\]
We call this algorithm naive as it assumes that $\widehat{P}_i^{(n)}$ is a reasonable estimator of ${P_i}^{(n)} := P_i(W^{(n)})$. Because the Voronoi partitions drift throughout the whole algorithm, this assumption is generally false.

However, the main issue with naive Lloyd's is not its naivet\'e. Rather, the issue lies with the idealized preconditioner $P_i(w)^{-1}$, which is poorly conditioned---it can become arbitrarily large. While this is not a problem in the noiseless setting, in the stochastic setting, the learning rate cannot become unbounded.
 

As a second pass, let us consider a second idealized online Lloyd's, where we introduce an upper bounding rate of $t_n^{-1}$ for some positive sequence $t_n$. Set the learning rate:
\[H_{\mathrm{ideal}',i}^{(n+1)} \leftarrow  \frac{\ind\{I^{(n+1)} = i\}}{\max\big\{nP_i^{(n)},\, t_n\big\}},\]
where we've refrained from preconditioning when $P_i(w) < t_n / n$. Note that if $t_n = o(n)$, then we can expect the set of points on which the algorithm will precondition to grow. Of course, this is idealized since we generally do not have direct access to $p$ with which to compute $P_i(w)$.


This motivates what we call the \emph{online Lloyd's algorithm}, which simultaneously constructs an estimator ${\widehat{P}_i}^{(n)}$ of ${P_i}^{(n)}$ based on the empirical rate at which the $i$th center has recently been updated in the past $s_n$ steps, for some sequence $s_n$. We define its learning rate by:
\begin{equation} \label{eqn:learning-rate-empirical}
H_i^{(n+1)} \leftarrow  \frac{\ind\{I^{(n+1)} = i\}}{\max\big\{n{\widehat{P}_i}^{(n)},\, t_n\big\}} \qquad\textrm{and}\qquad 
\widehat{P}_j^{(n)} = \frac{1}{s_n} \sum_{n_\circ\leq n' < n} \ind\{I^{(n' + 1)} = j\},
\end{equation}
where we denote $n_\circ = n - s_n$, and where $s_n$ and $t_n$ are non-decreasing sequences in $\mathbb{N}$. On the one hand, in order to obtain a low-bias estimator, we need $s_n = o(n)$ so that updates in the distant past are forgotten. But on the other, we would like the estimator to concentrate as $n$ goes to infinity, so we also require $s_n \uparrow \infty$. 

By introducing conditions on $s_n$ and $t_n$,  we show that ${\widehat{P}_i}^{(n)}$ is a consistent estimator of ${P_i}^{(n)}$ in \Cref{sec:lloyd}. Furthermore, we obtain the following convergence theorem, as a corollary of \Cref{thm:iterates-conv}.


\begin{restatable}[Convergence of iterates, online Lloyd's]{theorem}{lloydconvergence} \label{thm:lloydconvergence}
Let $H_j^{(n)}$ and $\widehat{P}_j^{(n)}$ as in (\ref{eqn:learning-rate-empirical}). Let $s_n$ and $t_n$ be non-decreasing sequences satisfying:
\begin{align*}\lim_{n\to\infty}\, \frac{n^{2/3} \log n}{s_n} = \lim_{n\to\infty} \, \frac{s_n \log s_n}{t_n} =  \lim_{n\to\infty}\,\frac{t_n}{n} = 0.\end{align*}
If $p$ is continuous, then $W^{(n)}$ globally converges to stationary points of the $k$-means cost $f$ almost surely.
\end{restatable}

